Security Issuance, Institutional Investors and Quid Pro Quo

Securities issuance through intermediaries is subject to agency problems and informational frictions. We examine these effects using SPAC data. We identify ``premium'' investors whose participation is linked to lower liquidation risk, higher returns, and lower redemption rates, consistent with both informational rents and agency frictions. In contrast, ``non-premium'' investors engage in non-agency quid pro quo relationships. Specifically, they receive high returns from an intermediary (quid) in exchange for a tacit agreement to participate in weaker future deals (quo). These relationships serve as insurance for issuers and intermediaries, enabling more issuers to access markets.

==> environment.tex <==
\usepackage{color,soul}  
\usepackage{tikz} 
\usepackage{url}
\usepackage{footmisc}
\usepackage{longtable}
\usepackage{amsmath,amsfonts,amssymb,amsthm}
\usepackage{mathtools}
\usepackage{enumerate}
\usepackage{siunitx}
\usepackage{amsmath,amssymb,amsthm}
\usepackage{graphicx}
\usepackage{placeins}
\usepackage{bigstrut}
\usepackage{indentfirst}
\usepackage{natbib}
\usepackage{verbatim}
\usepackage{multirow}
\usepackage{epstopdf}
\usepackage{adjustbox}
\usepackage[titletoc,title]{appendix}
\usepackage{setspace}
\doublespacing
% \onehalfspacing
\usepackage{bbm,bm}
\usepackage[left=1.00in, right=1.00in, top=1.00in, bottom=1.00in]{geometry}
\usepackage{color, colortbl}
\usepackage{import}
\usepackage{bbding}
\usepackage{multicol}
\usepackage[labelfont=bf,textfont=bf,]{caption}
\usepackage{graphicx, graphics}
\usepackage{booktabs, threeparttable, array}
\usepackage{rotating}
\usepackage{subcaption}

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\xmark}{\ding{55}}%

% New math commands
\newcommand{\sym}[1]{#1} % for symbols in Table
\newcommand{\E}{\mathbb{E}}
\newtheorem{hyp}{Hypothesis}

% CUSTOM COLORS FOR CITATION
\definecolor{sangre}{rgb}{0.6,0.18,0.19}
\definecolor{dullmagenta}{rgb}{0.4,0,0.4}
\definecolor{darkblue}{rgb}{0,0,0.6}
\ifx\pdfoutput\undefined
\usepackage[backref=none,hypertex,colorlinks,urlcolor = darkblue,citecolor = sangre,linkcolor=blue]{hyperref}
\else
\usepackage[backref=none,pdftex,hypertexnames=false,colorlinks,urlcolor = darkblue,citecolor =  sangre,linkcolor=blue]{hyperref}
% \usepackage[backref=page,pdftex,hypertexnames=false,colorlinks,urlcolor = darkblue,citecolor =  sangre,linkcolor=blue]{hype\fi

% LARGE HAT
\usepackage{scalerel,stackengine}
\stackMath
\newcommand\reallywidehat[1]{%
  \savestack{\tmpbox}{\stretchto{%
      \scaleto{%
        \scalerel*[\widthof{\ensuremath{#1}}]{\kern-.6pt\bigwedge\kern-.6pt}%
        {\rule[-\textheight/2]{1ex}{\textheight}}%WIDTH-LIMITED BIG WEDGE
      }{\textheight}% 
    }{0.5ex}}%
  \stackon[1pt]{#1}{\tmpbox}%
}
\parskip 1ex

% Theorem and Lemma Reference
% Theorem
\newtheorem{theorem}{Theorem}[subsection]
\renewcommand{\thetheorem}{\arabic{theorem}}% Remove subsection from theorem counter representation
% Corollary
\newtheorem{corollary}{Corollary}[theorem]
% Lemma
\newtheorem{lemma}{Lemma}
% Proposition
\newtheorem{proposition}{Proposition}[subsection]
\renewcommand{\theproposition}{\arabic{proposition}}% Remove subsection from theorem counter
% Definition
\newtheorem{definition}{Definition}[subsection]
\renewcommand{\thedefinition}{\arabic{definition}}% Remove subsection from theorem counter 
% Assumption
\newtheorem{assumption}{Assumption}[subsection]
\renewcommand{\theassumption}{\arabic{assumption}}% Remove subsection from theorem counter 

\newcommand{\Tau}{\mathcal{T}}

\usepackage{enumitem} % change itemize symbol
\usepackage{pifont}

%\usepackage{tabularray}
%\UseTblrLibrary{booktabs}

\newcommand\numberthis{\refstepcounter{equation}\tag{\theequation}}

\usepackage[capitalize]{cleveref} % cleveref needs to be loaded last
\setlength{\oddsidemargin}{0in}
\setlength{\evensidemargin}{0in}

% \usepackage[nomarkers,figuresonly]{endfloat} 
%\usepackage[nolists]{endfloat}
% \usepackage[nomarkers]{endfloat}

%%%% figure notes
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\newcommand\EightPtClose{\@setfontsize\EightPtClose\@viiipt{9}}
\newcommand\TenPtType{\@setfontsize\TenPtType\@xpt\@xiipt}
\def\notesize{\TenPtType}
\def\notesize{\EightPtClose}
\newenvironment{figurenotes}[1][Note]{\begin{minipage}[t]{\linewidth}\notesize{\itshape#1: }}{\end{minipage}}
\makeatother
%%%%%


% column centering
\usepackage{array}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
